The Luna Bound Propagator for Formal Analysis of Neural Networks

The parameterized CROWN analysis, a.k.a., alpha-CROWN has emerged as a practically successful abstract interpretation method for neural network verification. However, existing implementations of alpha-CROWN are limited to Python, which complicates integration into existing DNN verifiers and long-term production-level systems. We introduce Luna, a new abstract-interpretation-based bound propagator implemented in C++. Luna supports Interval Bound Propagation, the DeepPoly/CROWN analysis, and the alpha-CROWN analysis over a general computational graph. We describe the architecture of Luna and show that it outperforms the state-of-the-art alpha-CROWN implementation in terms of both bound tightness and computational efficiency on supported benchmarks from VNN-COMP 2025. Luna is publicly available at https://github.com/ai-ar-research/luna.

==> src/imgs/network.tex <==
\begin{figure}[t]
  \centering
  \begin{tikzpicture}[
    node distance=1.2cm and 2.2cm,
    neuron/.style={circle, draw=black, minimum size=20pt, inner sep=0pt, font=\small},
    hidden/.style={neuron, draw=black!60, fill=black!5},
    arr/.style={->, >=latex, thin, black!40},
  ]

    % Input layer
    \node[neuron] (i1) at (0, 2.4) {$x_1$};
    \node[neuron] (i2) at (0, 1.2) {$x_2$};
    \node[neuron] (i3) at (0, 0)   {$x_3$};

    % Hidden layer 1
    \node[hidden] (h11) at (2.5, 3.0) {};
    \node[hidden] (h12) at (2.5, 2.0) {};
    \node[hidden] (h13) at (2.5, 1.0) {};
    \node[hidden] (h14) at (2.5, 0.0) {};

    % Hidden layer 2
    \node[hidden] (h21) at (5.0, 2.6) {};
    \node[hidden] (h22) at (5.0, 1.4) {};
    \node[hidden] (h23) at (5.0, 0.2) {};

    % Output layer
    \node[neuron] (o1) at (7.5, 1.8) {$y_1$};
    \node[neuron] (o2) at (7.5, 0.6) {$y_2$};

    % Connections: input -> hidden 1
    \foreach \i in {1,2,3}
      \foreach \j in {1,2,3,4}
        \draw[arr] (i\i) -- (h1\j);

    % Connections: hidden 1 -> hidden 2
    \foreach \i in {1,2,3,4}
      \foreach \j in {1,2,3}
        \draw[arr] (h1\i) -- (h2\j);

    % Connections: hidden 2 -> output
    \foreach \i in {1,2,3}
      \foreach \j in {1,2}
        \draw[arr] (h2\i) -- (o\j);

    % Layer labels
    \node[font=\footnotesize, below=6pt] at (0,   -0.5) {Input};
    \node[font=\footnotesize, below=6pt] at (2.5, -0.5) {Layer $f_1$};
    \node[font=\footnotesize, below=6pt] at (5.0, -0.5) {Layer $f_2$};
    \node[font=\footnotesize, below=6pt] at (7.5, -0.5) {Output};

    % Top annotation
    \draw[->, >=latex, thin, black!50] (0, 3.8) -- (7.5, 3.8)
      node[midway, above, font=\footnotesize] {$N(\mathbf{x}) = f_2 \circ f_1(\mathbf{x})$};

  \end{tikzpicture}
  \caption{A layered feedforward neural network. Each layer $f_i$ applies an affine transformation followed by a non-linear activation function. Every node in one layer is connected to every node in the next, forming a fully connected architecture.}
  \label{fig:neural_network}
\end{figure}
